Experimental and Computational Investigation of the Influence of Ethanol on Auto-ignition of n-Heptane in Non-Premixed Flows

Experimental and computational investigations are carried out to elucidate the influence of ethanol addition on n-heptane auto-ignition in counterflows. An axisymmetric stream of air, temperature gradually increased, is directed onto the surface of an evaporating pool of a liquid fuel. The air-stream temperature at auto-ignition is measured at various strain rates for n-heptane, ethanol, and various n-heptane/ethanol mixtures. Critical conditions for auto-ignition are predicted employing San Diego Mechanism for both fuels and fuel mixtures, and the results are compared with measurements. Measurements and predictions show that low-temperature chemistry (LTC) plays a significant role in promoting auto-ignition of n-heptane at low strain rates, but there is insufficient residence time at high strain rates for LTC to take place, so auto-ignition is promoted by high-temperature chemistry. Experimental and computational results show addition of ethanol inhibits LTC of n-heptane. To identify the responsible elementary steps, computations are performed to identify those dominate O2 consumption and contribute to the temperature rise in the reaction zone for n-heptane and n-heptane/ethanol mixtures at low strain rates. For n-heptane, O2 is consumed primarily by the low-temperature steps that result in ketohydroperoxide; the temperature rise is produced by subsequent LTC steps. For the mixtures, a key step consuming O2 is O2 + CH3CHOH = HO2 + CH3CHO, and the heat release occurs through the classical high-temperature reaction mechanism. Thus, the inhibition of auto-ignition that is observed to occur when ethanol is added to n-heptane arises from the competition for O2 between this step and the LTC addition of O2 to the heptyl radical and to the radical arising from the subsequent isomerization, for n-heptane.

==> ref.tex <==
\subsection*{References}
\begin{itemize}
\item Liu et al 2021: The effect of ethanol on n-heptane oxidation was studied using the reactive molecular dynamics (RMD) method. With different ethanol concentrations, simulations were performed under fuel-rich conditions from 2000 −2500 K. The results showed that ethanol addition had little effect on the n-heptane oxidation rate. However, the presence of ethanol inhibited the formation of major species (e.g. Ethylene and Formaldehyde) in different ways. The amount of C2H4 during n-heptane oxidation was clearly greater than that during n-heptane/ethanol oxidation, indicating that the dissociation of ethanol (C2H5OH →C2H4 + H2O) was not an effective pathway to produce C2H4. Conversely, ethanol addition had a two-fold impact on CH2O formation at high temperatures. Ethanol promoted the formation of the C2H5O radical, which was the main intermediate to produce CH2O. However, ethanol addition reduced the amount of n-heptane in the system, lowered the rate of CH3 radical formation, and subsequently decreased CH2O formation, consistent with previous experiments.
\end{itemize}
